Knowledge Graph Question Answering via SPARQL Silhouette Generation

Knowledge Graph Question Answering (KGQA) has become a prominent area in natural language processing due to the emergence of large-scale Knowledge Graphs (KGs). Recently Neural Machine Translation based approaches are gaining momentum that translates natural language queries to structured query languages thereby solving the KGQA task. However, most of these methods struggle with out-of-vocabulary words where test entities and relations are not seen during training time. In this work, we propose a modular two-stage neural architecture to solve the KGQA task. The first stage generates a sketch of the target SPARQL called SPARQL silhouette for the input question. This comprises of (1) Noise simulator to facilitate out-of-vocabulary words and to reduce vocabulary size (2) seq2seq model for text to SPARQL silhouette generation. The second stage is a Neural Graph Search Module. SPARQL silhouette generated in the first stage is distilled in the second stage by substituting precise relation in the predicted structure. We simulate ideal and realistic scenarios by designing a noise simulator. Experimental results show that the quality of generated SPARQL silhouette in the first stage is outstanding for the ideal scenarios but for realistic scenarios (i.e. noisy linker), the quality of the resulting SPARQL silhouette drops drastically. However, our neural graph search module recovers it considerably. We show that our method can achieve reasonable performance improving the state-of-art by a margin of 3.72% F1 for the LC-QuAD-1 dataset. We believe, our proposed approach is novel and will lead to dynamic KGQA solutions that are suited for practical applications.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> sections/motivation.tex <==
\section{Motivation and Approach}

==> supplimentary.tex <==
\def\year{2022}\relax
%\documentclass[letterpaper]{article}
%\usepackage{aaai22}  % DO NOT CHANGE THIS
%\usepackage{times}  % DO NOT CHANGE THIS
%\usepackage{helvet}  % DO NOT CHANGE THIS
%\usepackage{comment}
%\usepackage{courier}  % DO NOT CHANGE THIS
%\usepackage[hyphens]{url}  % DO NOT CHANGE THIS
%\usepackage{graphicx} % DO NOT CHANGE THIS
%\urlstyle{rm} % DO NOT CHANGE THIS
%\def\UrlFont{\rm}  % DO NOT CHANGE THIS
%\usepackage{natbib}  % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
%\usepackage{caption} % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
%\DeclareCaptionStyle{ruled}{labelfont=normalfont,labelsep=colon,strut=off} % DO NOT CHANGE THIS
%\frenchspacing  % DO NOT CHANGE THIS
%\setlength{\pdfpagewidth}{8.5in}  % DO NOT CHANGE THIS
%\setlength{\pdfpageheight}{11in}  % DO NOT CHANGE THIS
%
% These are recommended to typeset algorithms but not required. See the subsubsection on algorithms. Remove them if you don't have algorithms in your paper.
%\usepackage{algorithm}
%\usepackage{algorithmic}

%\usepackage[hyperref]{emnlp2020}
%\usepackage{times}
%\usepackage{latexsym}
%\renewcommand{\UrlFont}{\ttfamily\small}
%\usepackage{graphicx}
%\usepackage{booktabs}
%\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amssymb}
%\usepackage{enumitem}
%\usepackage{tabularx}
%\usepackage{comment}
%\usepackage{appendix}
%\usepackage{multirow}
%\usepackage{dblfloatfix}
%\usepackage{xr} %added by Dinesh G
% This is not strictly necessary, and may be commented out,
% but it will improve the layout of the manuscript,
% and will typically save some space.
%\usepackage{zref-xr}
%\usepackage{xr-hyper} 
%\usepackage{hyperref} 
%\usepackage{microtype}
%\usepackage{siunitx}
%\aclfinalcopy % Uncomment this line for the final submission
%\def\aclpaperid{***} %  Enter the acl Paper ID here

%\setlength\titlebox{5cm}
% You can expand the titlebox if you need extra space
% to show all the authors. Please do not make the titlebox
% smaller than 5cm (the original size); we will check this
% in the camera-ready version and ask you to change it back.
%\setcounter{secnumdepth}{1} 
%\newcommand\BibTeX{B\textsc{ib}\TeX}
\title{Knowledge Graph Question Answering Via SPARQL Silhouette Generation \\ (Appendix)}
%\title{A Neuro-Symbolic Approach to KBQA via SPARQL Silhouette Generation}
%\title{A Neural Approach to KBQA via SPARQL Silhouette Generation}
%\title{A Neural Approach to KBQA via Sparql Silhouette Generation}
%\title{Can BERT Improve Relations in Neural Knowledge Base Question Answering system ?}
%\author{Sukannya Purkayastha \\
 % IIT Kharagpur / Address %line 1 \\
 % Affiliation / Address line 2 \\
 % Affiliation / Address line 3 \\
 % \texttt{email@domain} \\\And
  %Saswati Dana \\
  %IBM Research / Address line 1 \\
 % Affiliation / Address line 2 \\
  %Affiliation / Address line 3 \\
  %\texttt{email@domain} \\}
%\date{}
%\begin{document}
%\maketitle
%\section{Hyperparameters Tuning}\label{1stsection}
% \begin{itemize}
% \item Computing infrastructure: 2 
% Tesla v100 GPUs for training our seq2seq model.
% 1 Tesla GPU for training Graph Search Module.
% \item Hyper- parameters: Please refer to the Table \ref{table:hyper-param} for hyper-parameters used in our model.
% \item  We use accuracy on
% validation set as criterion for selecting hyperparameters for all our experiments.
% \end{itemize}
\newpage
\section{Appendix}

\section{Noise Simulator}
%---------------------------------------
\begin{figure}[h!]
\centering
\includegraphics[width=0.7\columnwidth]{./images/masking_A.pdf}
\caption{An illustrative example for Scenario `A': Noise-Free Linking. To align the surface forms of the entities/relations mentions in the given question text, we used word embedding as it offers higher alignment $F_1$. We used Falcon as a linker.} 
\label{mask_A}
\end{figure}
%---------------------------------------
%-------------------------------------------------
\begin{figure}[h!]
\centering
\includegraphics[width=0.9\columnwidth]{./images/masking_B.pdf}
\caption{An illustrative example for Scenario `B': Partly Noisy Linking. To align the surface forms of the entities/relations mentions in the given question text, we used exact match as well as string overlap based {\em Jaccard similarity} with a threshold of $0.7$. We used Falcon as a linker.} 
\label{mask_B}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-------------------------------------------------
%\section{Hyperparameters Tuning}
%--------------------------------
\begin{table*}[h!]
%\small
\centering
\setlength\tabcolsep{2pt}
\renewcommand{\arraystretch}{1.4}
%\begin{threeparttable}
\begin{tabular}{lrr}
\toprule
Hyperparameter &\parbox{2cm}{\centering Tuning Range} & \parbox{1cm}{\centering Best Value} \\
\midrule
$\eta$ for Stage-I        & [\num{0.1}, \num{0.2}, \num{0.25}, \num{0.50}] & $0.25$\\
$\eta$ for Stage-II  & [$10^{-4}$, $10^{-5}$, $10^{-6}$]           &   $10^{-5}$    \\
$b$ for both stages          & \num{8}                                        & \num{8} \\
$\alpha$ for LC-QuAD-1          & [\num{0.1}, \num{0.4}, \num{0.6}, \num{0.7}] & \num{0.4}  \\
$\alpha$ for QALD-9             & [\num{0.1}, \num{0.4}, \num{0.6}, \num{0.7}] & \num{0.6}      \\
\bottomrule
\end{tabular}
\caption{Tuning range and the final chosen best values of various hyperparameters. $\eta$ means learning rate and $b$ means batch size.}
\label{table:hyper-param}
\end{table*}
%----------------------------
%-----------------------------------
\begin{figure*}[h!]
\centering
%\includegraphics[width=1.3\columnwidth]{./images/CNN.pdf}
\includegraphics[width=1.5\columnwidth]{./images/valid_accuracy.pdf}
\caption{Change in validation set accuracy with hyperparameter $\alpha$}
\label{fig:val_accuracy}
\end{figure*}
%-----------------------------------
%-----------------------------

%--------------------------------
%----------------------------
\begin{figure*}[h!]
\centering
\includegraphics[width=2\columnwidth]{./images/Example.pdf}
\caption{An example of input to the neural graph search module.}
\label{input_graph_search}
\end{figure*}

\begin{comment}
\begin{table*}[h]
\centering
\setlength\tabcolsep{2pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llrr}
\toprule
Question & Entity & Predicted Relation & Gold Relation\\
\midrule
\parbox{0.50\textwidth}{Where was the person born who died in Bryn Mawr Hospital?}  & Byrn\_Mawr\_Hospital & deathPlace & placeOfDeath \\
\midrule
Name the rivers who originate from Essex? & Essex & sourceRegion & mouthPlace \\
\midrule
\parbox{0.50\textwidth}{Name the artist who made Dream Dancing and is often associated with Joe Pass}
& Joe\_Pass & associatedMusicalArtist & Karafarin\_Bank associatedBand \\
 
\midrule 
\parbox{0.50\textwidth}{What is used as money for French Southern and Antarctic Lands is also the  product of the Karafarin Bank ?}	
& products & product \\
\bottomrule
\end{tabular}
\caption{Examples Where Stage-II Graph Search Module Falling Short}
\label{failing_examples}
\end{table*}
\end{comment}
%\pagebreak
%-------------------------------------------
\begin{table*}[!b]%[h!]
\centering
\setlength\tabcolsep{8pt}
\renewcommand{\arraystretch}{1.8}
\begin{tabular}{lll}
\toprule
Question  &  \parbox{1.6cm}{Gold\\Relation}& \parbox{1.5cm}{Predicted Relation}\\
\midrule
\parbox{7.5cm}{Where was the person born who died in \textbf{Bryn Mawr Hospital}?}  & placeOfDeath & deathPlace \\
\midrule
\parbox{7.5cm}{ Name the rivers who originate from \textbf{Essex}?} & mouthPlace & sourceRegion\\
\midrule
\parbox{7.5cm}{Name the artist who made Dream Dancing and is often associated with \textbf{Joe Pass}.}
 & associatedBand   & associatedMusicalArtist\\
\midrule 
\parbox{7.5cm}{What is used as money for French Southern and Antarctic Lands is also the  product of the \textbf{Karafarin Bank} ?}	
 & product & products\\
\bottomrule
\end{tabular}
\caption{Anecdotal examples from LC-QuAD-1 test set where graph search module is unable to disambiguate between two closely related relations (gold and predicted) that are available for the highlighted entities in DBpedia.}
\label{failing_examples}
\end{table*}
%-------------------------------------------
%--------------------------------
\begin{table*}[h!]
\centering
\setlength\tabcolsep{9pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lll}
\toprule
Question & Gold SPARQL & SPARQL silhouette\\
\midrule
\parbox{0.18\textwidth}{Who was called Scarface?} & 

\parbox{0.38\textwidth}{SELECT ?uri 
 WHERE \\ 
 \{\\
 ?uri dbo:alias ?alias\\
 FILTER \textbf{contains(lcase(?alias),\\"scarface")}\\
 \}} &
\parbox{0.33\textwidth}{SELECT DISTINCT ?uri WHERE\\ 
\{\\ 
\;\;dbr:Scarface dbo:alias ?uri\\
\}}\\
\midrule

\parbox{0.18\textwidth}{Who was called Rodzilla?}
& \parbox{0.38\textwidth}{SELECT DISTINCT ?uri WHERE\\
\{\\
?uri \textbf{\textless  http://xmlns.com/foaf/0.1/nick\textgreater \\
``Rodzilla''@en}\\
\}} &  
\parbox{0.33\textwidth}{SELECT DISTINCT ?uri WHERE \\ 
\{\\ 
dbr:Rodzilla dbo:alias ?uri \\
\}}\\
\midrule 
\parbox{0.18\textwidth}{Give me all gangsters from the prohibition era.} & 

\parbox{0.38\textwidth}{SELECT DISTINCT ?uri WHERE \\ 
 \{\\
 ?uri dbo:occupation dbr:Gangster ; \\ \textbf{dct:subject} \textbf{dbc:Prohibition-eragangsters}\\
 \}} &
\parbox{0.33\textwidth}{SELECT   DISTINCT   ?uri   WHERE\\ 
\{\\ 
?uri   a   dbo:Film  ; \\ 
dbo:time dbr:Gangsters\_of\_the\_Frontier\\ \}}\\
\bottomrule

\end{tabular}
\caption{Anecdotal examples from QALD-9 test set where gold SPARQL have a peculiar structure just because the specific way in which the corresponding facts are present in the DBpedia.}
\label{atypical_examples}
\end{table*}


\begin{comment}
\parbox{0.18\textwidth}{Which artists were born on the same date as Rachel Stevens?}	
& 
\parbox{0.38\textwidth}{SELECT DISTINCT ?uri WHERE\\
\{\\
?uri \textbf{a} dbo:Artist  ;\\
 dbr:Rachel\_Stevens dbo:birthDate ?birthdate .\\
?uri dbo:birthDate ?birthdate\\
\}} & 
\parbox{0.33\textwidth}{SELECT DISTINCT ?uri WHERE\\
\{\\
dbr:Rachel\_Stevens  dbo:birthPlace ?uri\\
\}} \\
\midrule 
\parbox{0.18\textwidth}{Who was the father of Queen Elizabeth II?} & 
\parbox{0.38\textwidth}{SELECT DISTINCT * WHERE\\
\{\\
res:Elizabeth\_{II} dbo:parent ?uri .\\
?uri \textbf{\textless
http://xmlns.com/foaf/0.1/gender\textgreater\\``male''@en}\\
\}}  &
\parbox{0.33\textwidth}{SELECT DISTINCT ?uri WHERE\\
\{\\ 
   dbr:Elizabeth\_{II} dbo:parent ?uri\\
\}}\\

\midrule
\parbox{0.18\textwidth}{Which animals are critically endangered?} & 
\parbox{0.38\textwidth}{SELECT DISTINCT ?uri WHERE\\
\{\\
 ?uri \textbf{a} dbo:Animal; \\ dbo:conservationStatus \textbf{ `CR'}\\
\}}  &
\parbox{0.33\textwidth}{SELECT DISTINCT ?uri WHERE\\
\{\\ 
   dbr:Endangered\_Species\_(H.A.W.K.\_album) dbo:principal ?uri\\
\}}\\
\end{comment}


%-----------------------------------
%-------------------------

%-------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[h!]
\centering
\setlength\tabcolsep{7pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lll}
\toprule
Question & Gold SPARQL & SPARQL silhouette\\
\midrule
\parbox{0.18\textwidth}{Which countries have more than ten volcanoes?}
& \parbox{0.38\textwidth}{SELECT DISTINCT ?uri WHERE \\
\{\\
?x a dbo:volcano ; \\ dbo:locatedInArea ?uri .\\ ?uri a dbo:Country\\
\} \textbf{GROUP BY} ?uri HAVING\\ ( COUNT(?x) \textgreater 10 )\\
} &  
\parbox{0.33\textwidth}{SELECT DISTINCT ?uri WHERE \\ 
\{\\ 
?uri a dbo:Country ;\\ dbo:location dbr:Countries\_of\_the\_United\_Kingdom \\
\}}\\
\midrule 
\parbox{0.18\textwidth}{Give me a list of all critically endangered birds.}
& 
\parbox{0.38\textwidth}{SELECT DISTINCT ?uri ?p WHERE \\
\{\\
?uri rdf:type dbo:Bird \\\{ ?uri dbo:conservationStatus "CR" \} \\ \textbf{UNION} \{ ?uri dct:subject \\ dbc:Critically\_endangered\_animals \}\\
\}} & 
\parbox{0.33\textwidth}{SELECT DISTINCT ?uri WHERE\\
\{\\
?uri a dbo:Film ; \\
dbo:principal dbr:Endangered\_Species\_(H.A.W.K.\_album \\
\}} \\
\midrule 

\parbox{0.18\textwidth}{Which daughters of British earls died at the same place they were born at?
} & 
\parbox{0.38\textwidth}{SELECT DISTINCT ?uri WHERE\\
\{\\
?uri rdf:type yago:WikicatDaughtersOfBritishEarls ; \\ dbo:birthPlace ?x ; \\ dbo:deathPlace ?y \textbf{FILTER} ( ?x = ?y ) \\
\}}  &
\parbox{0.33\textwidth}{SELECT DISTINCT ?uri WHERE\\
\{\\ 
 ?uri rdf:type yago:WikicatStatesOfTheUnitedStates ; \\
 dbo:place dbr:Daughters\_of\_the\_Dust\\
\}}\\
\bottomrule

\end{tabular}
\caption{Anecdotal examples from QALD-9 test set where gold SPARQL comprises infrequent SPARQL keywords. The corresponding SPARQL Silhouette predicted by our Stage-I is also shown for these examples.}
\label{missing_for_less_freq_keyword}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{table}[t]
%\small
\centering
\setlength\tabcolsep{2.5pt}
\renewcommand{\arraystretch}{0.9}
%\begin{threeparttable}
\begin{tabular}{llrrrr}
\toprule
\parbox{0.5cm}{\centering Model Type} & \parbox{0.5cm}{\centering Model Name} &  AM   &   Prec.  &    Recall  & $F_1$  \\
\midrule
\multirow{3}*{\parbox{1.2cm}{\centering Stage-I (Transformer)}} & No Noise	&	 $77.58$    &   $77.82$   &   $77.78$   &   $77.79$  \\
& Part Noise   & 	 $34.73$    &   $35.87$   &   $35.92$   &   $35.89$ \\
& Full Noise    & $20.72$    &   $21.49$   &   $21.43$   &   $21.46$ \\
\bottomrule
\end{tabular}
\caption{Test set performance on {LC-QuAD-1} dataset when Transformer is used in Stage I.}
%Stage-II numbers are under full noise scenario. 
%QAmp is the top entry of \texttt{LC-QuAD-1} leader board \cite{vakulenko2019message}.
 
\label{table:lcquad_transformer}
\end{table}
\end{comment}

\section{Evaluation Metric}\label{eval_met}

{\em 1) Precision, Recall, and $F_1$ for Single Question:} For single question $Q$, we compute precision $P$, recall $R$, and $F_1$ using the set of {\em gold answer entities} $S_g$ and {\em predicted answer entities} $S_p$. 
While computing these metrics, we handle boundary cases as follows. If $S_g=S_p=\emptyset$ then we take $P=R=F_1=1$. If only $S_g=\emptyset$ then we take $R=F_1=0$.\\
{\em 2) Macro Precision, Macro Recall, Macro $F_1$, and Macro $F_1$ QALD:}
These metrics are defined for the whole dataset. For this, we first compute $P$, $R$, and $F_1$ at individual question level and average of these numbers across entire dataset gives us the {\em macro} version of these metrics. For $F_1$, if use the boundary condition of having $P=1$ when $S_p=\emptyset, S_g\neq \emptyset$ then such a Macro $F_1$ is called as {\em Macro $F_1$ QALD} as per \citet{ngomo20189th}. But if we instead use $P=0$ then it is called Macro $F_1$.\\
{\em 3) Precision, Recall, and $F_1$ for the whole set:} For whole set, $P$ and $R$ are same as {\em macro} version of these metrics. $F_1$, however, is computed by taking Harmonic mean of these $P$ and $R$. The reported metrics for the {LC-QuAD-1} dataset were computed in this manner.\\ 
{\em 4) Answer Match (AM):} For a question $Q$, when executing the predicted SPARQL, if we have $S_p=S_g$ then we say AM=1 otherwise AM=0.\\
\begin{comment}
{\em 5) Accuracy for Stage-II:} We measure  performance of Stage-II as follows. Let $N$ be the total number of triples across all the generated {SPARQL} silhouette such that one of the entity (subject or object) in this triple is correct. After passing through neural graph search module, let $N_c$ be the number of these triples whose relation is found to be correct. Then we call $N_c/N$ as {\em accuracy} of the Stage-II. 
\end{comment}
%\section{Performance of transformers}
\begin{comment}
\begin{table}[t!]
%\small
\centering
\setlength\tabcolsep{2.5pt}
\renewcommand{\arraystretch}{0.9}
%\begin{threeparttable}
\begin{tabular}{llrrrr}
\toprule
\parbox{0.5cm}{\centering Model Type} & \parbox{0.5cm}{\centering Model Name} &  AM   &   Prec.  &    Recall  & $F_1$  \\
\midrule
\multirow{3}*{\parbox{1.2cm}{\centering Stage-I (Transformer)}} & No Noise	&	 $77.58$    &   $77.82$   &   $77.78$   &   $77.79$  \\
& Part Noise   & 	 $34.73$    &   $35.87$   &   $35.92$   &   $35.89$ \\
& Full Noise    & $20.72$    &   $21.49$   &   $21.43$   &   $21.46$ \\
\bottomrule
\end{tabular}
\caption{Test set performance on {LC-QuAD-1} dataset when Transformer is used in Stage I.}
%Stage-II numbers are under full noise scenario. 
%QAmp is the top entry of \texttt{LC-QuAD-1} leader board \cite{vakulenko2019message}.
 
\label{table:lcquad_transformer}
\end{table}
\end{comment}



\section{Anecdotal Examples}\label{appen:anecdotal_examples}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Anecdotal Examples}
Table \ref{failing_examples} shows examples from LC-QuAD-1 test set where our neural graph search module is unable to disambiguate between two very similar looking relations that exist in DBpedia for an entity.

Table \ref{atypical_examples} captures examples from QALD-9 test set where gold SPARQL have a peculiar structure just because the way in which corresponding facts are being captured within in the DBpedia and that makes it almost impossible for any KB agnostic techniques (such as seq2seq) to output such structures. The first two rows of Table \ref{failing_examples} shows examples where gold SPARQL queries of two very similar questions is quite different. Even though Falcon picks correct entities, our SPARQL silhouette struggle to yield two differently structured SPARQL queries for two very similar looking natural language questions. Third row of the table contains some entities/relations containing \textit{dct, dbc}, etc. Falcon linker does not tag these kinds of entity/relation, so we miss out correctly predicting the sketch in Stage-I and so in Stage-II as well. 

Table \ref{missing_for_less_freq_keyword} shows various examples from QALD-9 test set where we miss predicting the correct sketch of SPARQL because of very few number of such examples present in the training set. These are examples where SPARQL contains infrequent keywords such as GROUP BY, UNION, FILTER etc.
%\input{./sections/appendix.tex}
% \bibliographystyle{acl_natbib}
% \bibliography{all}
%\end{document}

